Efficient and Tunable Photochemical Charge Transfer via Long-Lived Bloch Surface Wave Polaritons

Achieving precise control of photoinduced molecular charge transfer reactions underpins key emerging technologies. As such, the use of hybrid light-matter molecular exciton-polariton states has been proposed as a scheme to directly modify the efficiency and rate of such reactions. However, the efficacy of polariton-driven photochemistry remains an open question. Here, we demonstrate conditions under which photoinduced polaritonic charge transfer can be achieved and directly visualized using momentum resolved ultrafast spectroscopy. Key conditions for charge transfer are satisfied using Bloch surface wave polaritons, which exhibit favorable dispersion characteristics that permit the selective pumping of hybrid states with long lifetimes (100-400 fs) that permit vibrationally assisted molecular charge transfer. Using this approach, we tune the energetic driving force for charge separation, reducing it by as much as 0.5 eV compared to the bare exciton. These results establish that tunable and efficient polariton-driven molecular charge transfer is indeed possible using carefully considered photonic systems.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
